Federated Over-Air Subspace Tracking from Incomplete and Corrupted Data

In this work we study the problem of Subspace Tracking with missing data (ST-miss) and outliers (Robust ST-miss). We propose a novel algorithm, and provide a guarantee for both these problems. Unlike past work on this topic, the current work does not impose the piecewise constant subspace change assumption. Additionally, the proposed algorithm is much simpler (uses fewer parameters) than our previous work. Secondly, we extend our approach and its analysis to provably solving these problems when the data is federated and when the over-air data communication modality is used for information exchange between the $K$ peer nodes and the center. We validate our theoretical claims with extensive numerical experiments.

==> arxiv_sims.tex <==

%\clearpage

\begin{figure*}[t!]
\centering
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=2 by 1,
            horizontal sep=3cm,
            vertical sep=1cm,
                        x descriptions at=edge bottom,
            %y descriptions at=edge left,
        },
        % load the style created in the preamble
        %my stylecompare,
                %ymin=1e-15, ymax=0,
        enlargelimits=false,
        width = .45\linewidth,
        height=4.5cm,
        enlargelimits=false,
                grid=both,
    grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
    minor x tick num=5,
    minor y tick num=5,
    ]
       \nextgroupplot[
%		legend entries={
%					simple PCA,
%					NORST,
%					NORST-nodet,
%					PETRELS,
%					GROUSE,
%					%Fed-ST-Miss,
%            		%NORST-sliding[$\beta=1$ $R=0$] ($7$ms),
%            		%NORST-sliding[$\beta=10$ $R=1$] ($11$ms),            		
%            		%PETRELS ($29$ms),
%            		},
%            legend style={at={(2.5, 1.3)}},
%            %legend style={at={(1,1.8)}}, % use this if one column fig
%            legend columns = 4,
%            legend style={font=\footnotesize},
			%ymode=log,
            xlabel={\small{Mini-batch index ($j$)}},
            ylabel={{$\SE(\Phat_{j},\P_j)$}},
                        title style={at={(0.5,-.35)},anchor=north,yshift=1},
            title={\small{(a) Small rotations at each time}},
            %xtick={300, 1000, 1700, 2400},
            %xticklabels={$300$, $1000$, $1700$, $2400$},
                        xticklabel style= {font=\footnotesize, yshift=-1ex},
            yticklabel style= {font=\footnotesize, xshift=0ex},
        ]
%			\addplot [black, line width=1.2pt, mark=Mercedes star,mark size=6pt, mark repeat=1] table[x index = {0}, y index = {1}, select coords between index={0}{24}]{\stmiss};
	        %\addplot [black, dotted,  line width=1.2pt, mark=square,style=solid,mark size=3pt, mark repeat=1] table[x index = {2}, y index = {3}]
	        %{\pwjustall};
	        %\addplot [black, line width=1.2pt, mark=diamond, style=solid, mark size=5pt, mark repeat=1] table[x index = {4}, y index = {5}]
	        %{\pwjustall};
			\addplot [black, line width=1.2pt, mark=Mercedes star,mark size=6pt, mark repeat=2] table[x index = {0}, y index = {3}]{\smallrot};
			\addplot [olive, line width=1.2pt, mark=o,mark size=4pt, mark repeat=2] table[x index = {0}, y index = {1}]{\smallrot};
	        %\addplot [olive, dotted,  line width=1.2pt, mark=square,style=solid,mark size=3pt, mark repeat=1] table[x index = {8}, y index = {9}]
	        %{\pwjustall};
	        %\addplot [olive, line width=1.2pt, mark=diamond,style=solid,mark size=5pt, mark repeat=1] table[x index = {10}, y index = {11}]
	        %{\pwjustall};

			\addplot [teal, line width=1.2pt, mark=diamond,mark size=5pt, mark repeat=2] table[x index = {0}, y index = {2}]{\smallrot};
			\addplot [red, line width=1.2pt, mark=triangle,mark size=4pt, mark repeat=2] table[x index = {0}, y index = {1}]{\smallrotcomp};
	        %\addplot [olive, dotted,  line width=1.2pt, mark=square,style=solid,mark size=3pt, mark repeat=1] table[x index = {8}, y index = {9}]
	        %{\pwjustall};
	        %\addplot [olive, line width=1.2pt, mark=diamond,style=solid,mark size=5pt, mark repeat=1] table[x index = {10}, y index = {11}]
	        %{\pwjustall};

			\addplot [orange, line width=1.2pt, mark=square,mark size=5pt, mark repeat=2] table[x index = {0}, y index = {2}]{\smallrotcomp};

%				        	        \addplot [blue, line width=1.6pt, mark=oplus,mark size=3pt] table[x index = {18}, y index = {19}]{\stmiss};


\nextgroupplot[
		legend entries={
					simple-PCA,
					NORST,
					STMiss-nodet,
					PETRELS,
					GROUSE,
					%Fed-ST-Miss,
            		%NORST-sliding[$\beta=1$ $R=0$] ($7$ms),
            		%NORST-sliding[$\beta=10$ $R=1$] ($11$ms),            		
            		%PETRELS ($29$ms),
            		},
            legend style={at={(0.5, 1.3)}},
            %legend style={at={(1,1.8)}}, % use this if one column fig
            legend columns = 5,
            legend style={font=\footnotesize},
			ymode=log,
            xlabel={\small{Mini-batch index $j$}},
            ylabel={{$\SE(\Phat_{j},\P_j)$}},
                        title style={at={(0.5,-.35)},anchor=north,yshift=1},
            title={\small{(b) Piecewise Constant Subspace  -- Large}},
            %xtick={300, 1000, 1700, 2400},
            %xticklabels={$300$, $1000$, $1700$, $2400$},
                        xticklabel style= {font=\footnotesize, yshift=-1ex},
            yticklabel style= {font=\footnotesize, xshift=-.5ex},
        ]

			\addplot [black, line width=1.2pt, mark=Mercedes star,mark size=6pt, mark repeat=2] table[x index = {0}, y index = {3}]{\pwconst};
			\addplot [olive, line width=1.2pt, mark=o,mark size=4pt, mark repeat=2] table[x index = {0}, y index = {1}]{\pwconst};
			\addplot [teal, line width=1.2pt, mark=diamond,mark size=5pt, mark repeat=2] table[x index = {0}, y index = {2}]{\pwconst};
			\addplot [red, line width=1.2pt, mark=triangle,mark size=4pt, mark repeat=1] table[x index = {6}, y index = {7}, select coords between index={0}{24}]{\stmiss};
	        %\addplot [olive, dotted,  line width=1.2pt, mark=square,style=solid,mark size=3pt, mark repeat=1] table[x index = {8}, y index = {9}]
	        %{\pwjustall};
	        %\addplot [olive, line width=1.2pt, mark=diamond,style=solid,mark size=5pt, mark repeat=1] table[x index = {10}, y index = {11}]
	        %{\pwjustall};

			\addplot [orange, line width=1.2pt, mark=square,mark size=5pt, mark repeat=1] table[x index = {12}, y index = {13}, select coords between index={0}{24}]{\stmiss};


%       \nextgroupplot[
%			ymode=log,
%            xlabel={\small{Mini-batch index $j$}},
%            %ylabel={{$\SE(\Phat_{j},\P_j)$}},
%                        title style={at={(0.5,-.35)},anchor=north,yshift=1},
%            title={\small{(c) Piecewise Constant Subspace  -- Small}},
%            %xtick={300, 1000, 1700, 2400},
%            %xticklabels={$300$, $1000$, $1700$, $2400$},
%                        xticklabel style= {font=\footnotesize, yshift=-1ex},
%            yticklabel style= {font=\footnotesize, xshift=.5ex},
%        ]
%			\addplot [black, line width=1.2pt, mark=Mercedes star,mark size=6pt, mark repeat=2] table[x index = {0}, y index = {3}]{\newgenlarge};
%			\addplot [olive, line width=1.2pt, mark=o,mark size=4pt, mark repeat=2] table[x index = {0}, y index = {1}]{\newgenlarge};
%			\addplot [teal, line width=1.2pt, mark=diamond,mark size=5pt, mark repeat=2] table[x index = {0}, y index = {2}]{\newgenlarge};


    \end{groupplot}
\end{tikzpicture}
%\vspace{-.5cm}
\caption{\small{Comparison of ST-Miss Algorithms in the centralized setting.}}
\vspace{-.7cm}
\label{fig:st_miss}
\end{figure*}


\Section{Numerical Experiments}\label{sec:sims}
%Experiments are performed on a Desktop Computer with Intel$^{\textsuperscript{\textregistered}}$ Xeon $8$-core CPU with $32$GB RAM and the results are averaged over $100$ independent trials. 
The codes are available at \url{https://github.com/praneethmurthy/distributed-pca}.


\subsection{Centralized STMiss}
\subsubsection{Small Rotations at each time} We first consider the centralized setting for Subspace Tracking with missing data (Sec. \ref{sec:stmiss}). We demonstrate results under two sets of subspace change models. First we consider the ``rotation model'' that has been commonly used in the literature \cite{petrels, grouse_global}.  At each time $t$, we generate a $n \times r$ dimensional subspace $\P_{(t)} = e^{-\delta_t B_t} \P_{(t-1)} $ with $\P_{(0)}$ generated by orthonormalizing the columns of a i.i.d. standard Gaussian matrix and $B_t$ is some skew symmetric matrix to simulate rotations and $\delta_t$ controls the amount of rotation (for this experiment we set $\delta_t = 10^{-4}$ which ensures that $\Delta_{tv} \approx 10^{-2}$). We generate matrix $\tilde{A}$ as a i.i.d. uniform random matrix of size $r \times \tmax$ and set the $t$-th column of the true data matrix $\tl_t = \P_{(t)} \tilde{\at}_t$. Thus, in the notation of our result, $\P_j$ is the matrix of the top $r$ left singular vectors of $\tL_j = [\tl_{(j-1)\alpha + 1} , \cdots \tl_{j\alpha}]$ and $\A_j = \P_j^\top \tL_j$. In all experiments, we choose $n=1000$ and $d = 3000$. We simulate the set of observed entries using a bernoulli model where each element of the matrix is observed with probability $0.9$. For all experiments, we set $r = 30$ and the fraction of missing entries to be $0.1$. We implement STMiss-nodet (Algorithm \ref{algo:norst_nodet}) and set $r = 30$. We compare with NORST \cite{rrpcp_tsp19} (the state-of-the-art theoretically), GROUSE \cite{grouse_global}, and PETRELS \cite{petrels} (the state-of-the-art experimentally). For all algorithms, we used default parameters mentioned in the codes. We also implement the simple PCA method wherein we estimate $\Phat_j$ as the top-$r$ left singular vectors of $\Y_j$ for each mini-batch. For all algorithms, the mini-batch size was chosen as $\alpha = 60$. The results are shown in Fig. \ref{fig:st_miss}(a). We see that as specified by Theorem \ref{thm:naive}, the simple PCA algorithm does not improve the recovery errors since it is not exploiting slow subspace change. However, all other algorithms exploit slow-subspace change and thus are able to provide better estimates with time. We also notice that PETRELS is the fastest to converge, followed by NORST and STMiss-nodet, and finally GROUSE. This is consistent with the previous set of results in \cite{rrpcp_tsp19}.


\subsubsection{Piecewise Constant}
Next, we consider a piecewise constant subspace change model that has been considered in the provable subspace tracking literature \cite{rrpcp_tsp19}. In this, we simulate a large subspace change at $t_1 = 1500$. The subspace is fixed until then, i.e., $\P_j = \P_1$ for all $j \in [1, \lceil t_1/\alpha \rceil)$ and $\P_j = \P_2 $ for all $j \in [\lceil t_1/\alpha \rceil, \lceil \tmax/\alpha \rceil]$. The results are shown in Fig. \ref{fig:st_miss}(b). Notice that NORST and STMiss-nodet significantly outperform simple PCA as both exploit slow subspace change. Additionally, even though the change is large (in the notation of Definition \ref{def:large_ss} given in the supplementary material, $\Delta_{\mathrm{large}} \approx 1$  and $\Delta_{tv} = 0$), STMiss-nodet is also able to adapt without requiring a detection step. Finally, since the updates are always improving, after a certain time, NORST stops improving the subspace estimates, but STMiss-nodet improves it and gets a better result. 


%\subsubsection{Piecewise Constant for Small Time}
%Finally, we consider a setting that is easier than the first setting, but harder than the second setting. We generate $\P_j$'s for each $j in \J_j$ fo length $\alpha$, and use the rotation model such that $\Delta_{tv} \approx 1$. As predicted by Theorem \ref{thm:naive} and Theorem \ref{thm:central_timevar}, the simple PCA (naive) method works better than the NORST and NORST-nodet algorithms. 


%We do not compare with other STmiss methods since \cite{rrpcp_tsp19} contains an extensive numerical experiment section that shows that under the settings considered in this paper, NORST \cite{rrpcp_tsp19} is comparable to PETRELS \cite{petrels}.

\subsection{Fedrated ST-Miss}
We also implement Algorithm \ref{algo:fed_nodet_given_init} to corroborate our theoretical claims. We use the exact data generation method as we did in the centralized setting. To simulate over-air communication, we replace the inbuilt \texttt{SVD} routine of matlab by a power method code snippet, and by adding iteration noise. In each iteration, we add i.i.d. Gaussian noise with variance $10^{-6}$. The results are presented in Fig. \ref{fig:fed_st_miss}. Notice that in both cases, Algorithm \ref{algo:fed_nodet_given_init} works as well as NORST even though NORST cannot deal with iteration noise. Additionally, as opposed to the centralized setting (Fig. \ref{fig:st_miss}(b)), the error of Fed-OA-RSTMiss-nodet in Fig. \ref{fig:fed_st_miss} does not improve beyong the iteration noise level of $10^{-6}$. 


\begin{figure*}[t!]
\centering
\begin{tikzpicture}
    \begin{groupplot}[
        group style={
            group size=3 by 1,
            horizontal sep=2cm,
            vertical sep=1cm,
                        x descriptions at=edge bottom,
            %y descriptions at=edge left,
        },
        % load the style created in the preamble
        %my stylecompare,
                %ymin=1e-15, ymax=0,
        enlargelimits=false,
        width = .4\linewidth,
        height=4.5cm,
        enlargelimits=false,
                grid=both,
    grid style={line width=.1pt, draw=gray!10},
    major grid style={line width=.2pt,draw=gray!50},
    minor x tick num=5,
    minor y tick num=5,
    ]
       \nextgroupplot[
			%ymode=log,
            xlabel={\small{Mini-batch index ($j$)}},
            ylabel={{$\SE(\Phat_{j},\P_j)$}},
                        title style={at={(0.5,-.35)},anchor=north,yshift=1},
            title={\small{(a) Small rotations at each time}},
            %xtick={300, 1000, 1700, 2400},
            %xticklabels={$300$, $1000$, $1700$, $2400$},
                        xticklabel style= {font=\footnotesize, yshift=-1ex},
            yticklabel style= {font=\footnotesize, xshift=0ex},
        ]
%			\addplot [black, line width=1.2pt, mark=Mercedes star,mark size=6pt, mark repeat=1] table[x index = {0}, y index = {1}, select coords between index={0}{24}]{\stmiss};
	        %\addplot [black, dotted,  line width=1.2pt, mark=square,style=solid,mark size=3pt, mark repeat=1] table[x index = {2}, y index = {3}]
	        %{\pwjustall};
	        %\addplot [black, line width=1.2pt, mark=diamond, style=solid, mark size=5pt, mark repeat=1] table[x index = {4}, y index = {5}]
	        %{\pwjustall};
			\addplot [black, line width=1.2pt, mark=Mercedes star,mark size=6pt, mark repeat=2] table[x index = {0}, y index = {3}]{\smallrotfed};
			\addplot [olive, line width=1.2pt, mark=o,mark size=4pt, mark repeat=2] table[x index = {0}, y index = {1}]{\smallrotfed};
	        %\addplot [olive, dotted,  line width=1.2pt, mark=square,style=solid,mark size=3pt, mark repeat=1] table[x index = {8}, y index = {9}]
	        %{\pwjustall};
	        %\addplot [olive, line width=1.2pt, mark=diamond,style=solid,mark size=5pt, mark repeat=1] table[x index = {10}, y index = {11}]
	        %{\pwjustall};

			\addplot [blue, line width=1.2pt, mark=diamond,mark size=5pt, mark repeat=2] table[x index = {0}, y index = {2}]{\smallrotfed};
%				        	        \addplot [blue, line width=1.6pt, mark=oplus,mark size=3pt] table[x index = {18}, y index = {19}]{\stmiss};


       \nextgroupplot[
       legend entries={
					simple PCA,
					NORST,
					Fed-OA-RSTMiss-nodet,
					PETRELS,
					GROUSE,
					%Fed-ST-Miss,
            		%NORST-sliding[$\beta=1$ $R=0$] ($7$ms),
            		%NORST-sliding[$\beta=10$ $R=1$] ($11$ms),            		
            		%PETRELS ($29$ms),
            		},
            legend style={at={(0.3, 1.3)}},
            %legend style={at={(1,1.8)}}, % use this if one column fig
            legend columns = 5,
            legend style={font=\footnotesize},
			ymode=log,
            xlabel={\small{Mini-batch index $j$}},
            %ylabel={{$\SE(\Phat_{j},\P_j)$}},
                        title style={at={(0.5,-.35)},anchor=north,yshift=1},
            title={\small{(b) Piecewise Constant Subspace  -- Large}},
            %xtick={300, 1000, 1700, 2400},
            %xticklabels={$300$, $1000$, $1700$, $2400$},
                        xticklabel style= {font=\footnotesize, yshift=-1ex},
            yticklabel style= {font=\footnotesize, xshift=-.5ex},
        ]
			\addplot [black, line width=1.2pt, mark=Mercedes star,mark size=6pt, mark repeat=2] table[x index = {0}, y index = {3}]{\pwconstfed};
			\addplot [olive, line width=1.2pt, mark=o,mark size=4pt, mark repeat=2] table[x index = {0}, y index = {1}]{\pwconstfed};
			\addplot [blue, line width=1.2pt, mark=diamond,mark size=5pt, mark repeat=2] table[x index = {0}, y index = {2}]{\pwconstfed};
			%\addplot [red, line width=1.2pt, mark=triangle,mark size=4pt, mark repeat=1] table[x index = {6}, y index = {7}, select coords between index={0}{24}]{\stmiss};
	        %\addplot [olive, dotted,  line width=1.2pt, mark=square,style=solid,mark size=3pt, mark repeat=1] table[x index = {8}, y index = {9}]
	        %{\pwjustall};
	        %\addplot [olive, line width=1.2pt, mark=diamond,style=solid,mark size=5pt, mark repeat=1] table[x index = {10}, y index = {11}]
	        %{\pwjustall};

			%\addplot [orange, line width=1.2pt, mark=square,mark size=5pt, mark repeat=1] table[x index = {12}, y index = {13}, select coords between index={0}{24}]{\stmiss};


    \end{groupplot}
\end{tikzpicture}
%\vspace{-.5cm}
\caption{\small{Corroborating the claims of Theorem \ref{thm1_newnorst}.}}
\vspace{-.7cm}
\label{fig:fed_st_miss}
\end{figure*}

% We generate the low-rank matrix this way without loss of generality since this allows us implicitly obtain the noise, $\V_j$ as well. We then implement the classical NORST algorithm, NORST-nodet (Algo 1) and the simple PCA algorithm. For all algorithms, we provide the value of the true rank, in these experiments it is $r = 30$, and we set the size of the mini-batch $\alpha = 60$. for the classical NORST, the number of subspace update steps is set to $25$. We set $\delta_t = \delta = 10^{-4}$ that ensures that $\SE(P_{(t-1)}, \P_{(t)}) \approx 10^{-2}$. We present the results in Fig. \ref{fig:small_rot}. 
%
%We demonstrate the efficacy of our result under two setting of subspace change. In the first experiment, we generate data as follows. 


% and the error is bounded by our choice of $\alpha$ and the ''noise''. We observed that inceasing $\alpha$ while keeping all other parameters fixed reduces the value of the error, but nonetheless, the error stays roughly the same. 

%\begin{figure}[t!]
%\centering
%\includegraphics[scale=.5]{figures/small_rot.jpg}id
%\caption{Small changes at each time}
%\label{fig:small_rot}
%\end{figure}
%
%
%To analyse the effect of $\delta_t$, we increased it to $10^{-2}$ and thus $\SE(\P_{(t-1)}, \P_{(t)}) \approx 0.2$, and in this case all algorithms fail (the scale is very small and thus it is misleading to think simple PCA is better than other algorithms. The results are given in Fig. \ref{fig:large_rot}. 
%
%\begin{figure}[t!]
%\centering
%\includegraphics[scale=.5]{figures/large_rot.jpg}
%\caption{Large changes at each time}
%\label{fig:large_rot}
%\end{figure}



%\begin{figure}[t!]
%\centering
%\includegraphics[scale=.5]{figures/large_drastic.jpg}
%\caption{Large and abrupt change at $t = 1500$.}
%\label{fig:large_drast}
%\end{figure}
%
%
%
%\begin{figure}[t!]
%\centering
%\includegraphics[scale=.5]{figures/new_genmodel_large.jpg}
%\caption{Large change every $\alpha$ frames.}
%\label{fig:large_newmodel}
%\end{figure}

%However, using the same model as above but with $\SE(\P_{j-1}, \P_j) \approx 0.2$, we get the following result. Notice that again, both NORST and NORST-nodet outperform the simple PCA method. 

%\begin{figure}[t!]
%\centering
%\includegraphics[scale=.5]{figures/new_genmodel_small.jpg}
%\caption{Small change every $\alpha$ frames.}
%\label{fig:small_newmodel}
%\end{figure}








%%\newcommand{\V}{\bm{V}}
%\subsubsection{Federated Power Method}
%Consider FedPM. We generate the data as follows: We set $n = 1000$, $r = 50$ and $\X = \U \Lambda \V^T + \U_{\perp} \Lambda_{\perp} \V_{\perp}^T$ with $\U^* = [\U, \U_{\perp}]$, $\V^* = [\V, \V_{\perp}]$ being orthonormal matrices. We then set $\Y = \X \X^T$ and try to estimate $\U$. At each iteration we generate channel noise as i.i.d. Gaussian r.v's with variance $\sigma_c^2$. %In all figures, we plot $\SE(\hat{\bm Q}_{l}, \U)$ v.s. $l$. 
%
%
%
%First we illustrate the claims of Lemma \ref{lem:desc} and show that choosing a larger value of $\taubatch$ indeed increases robustness to noise. We set $R = 0.91$, and consider $\taubatch = 1,10$ and $\sigma_c = 10^{-4}, 10^{-8}$. Notice from Fig. \ref{fig:fed_pm_sig} that increasing $\taubatch$ has a similar effect as that of reducing $\sigma_c$ (the $\taubatch =10, \sigma_c = 10^{-8}$ plot overlaps with $\taubatch = 1, \sigma_c=10^{-8}$). We also study the effect of varying the gap, $R = \{0.91, 0.30\}$ and observed that choosing a smaller value of $R$ helps us achieve exponentially faster convergence, while also letting us obtain a better estimate of $\U$ as indicated by Theorem \ref{thm:main_res}. 
%
%
%\subsubsection{Federated ST-Miss}
%Here we illustrate the performance of Algorithm \ref{algo:stmiss_dyn}. We generate the data as done in most subspace tracking literature. We set $\l_i = \P_j \at_i$ with {\em one subspace change} at $t = t_1 = 1500$. We generate $\P_1$ and $\P_2$ by orthonormalizing a standard Gaussian matrix of size $n \times r$ with $n = 1000$ and $r =30$. The entries of $\at_i$ are chosen i.i.d. from a uniform distribution, $\mathcal{U}[-1,1]$. Thus, all assumptions of Theorem \ref{thm:stmiss} as satisfied. We do not generate modeling noise in this experiment ($\bv_i = 0$). For the implementation of Algorithm \ref{algo:stmiss_dyn}, we additionally simulate channel noise, $\W_l \sim \mathcal{N}(0, \sigma_c^2)$ with $\sigma_c = 10^{-6}$. We compare the proposed method with $3$ state-of-the-art (centralized) methods for ST-Miss: NORST \cite{rrpcp_tsp19}, PETRELS \cite{petrels}, and GROUSE \cite{grouse_global}. 
%
%%\section{Exrta Details for Numerical Experiments}\label{app:sims}
%
%
%We implemented Algorithm \ref{algo:stmiss_dyn} with $\alpha = C f^2 r \log n = 60$, $\lthres = 2 \epsilon^2 \lambda^+ = 7 \times 10^{-4}$, $T = 25$. Notice that our algorithm converges to the noise level (channel noise) whereas NORST and PETRELS are able to track the subspace to approximately $10^{-12}$. GROUSE has a slower convergence (since this is a first order method) and thus it also tracks to only $10^{-6}$. As can be seen from Fig. \ref{fig:st_miss}, all algorithms are able to satisfactorily track the underlying subspace while PETRELS has the best performance. Despite the addition of channel noise, our method is comparable to GROUSE. 
%

